An Optimal $3$-Fault-Tolerant Connectivity Oracle

We present an optimal oracle for answering connectivity queries in undirected graphs in the presence of at most three vertex failures. Specifically, we show that we can process a graph $G$ in $O(n+m)$ time, in order to build a data structure that occupies $O(n)$ space, which can be used in order to answer queries of the form "given a set $F$ of at most three vertices, and two vertices $x$ and $y$ not in $F$, are $x$ and $y$ connected in $G\setminus F$?" in constant time, where $n$ and $m$ denote the number of vertices and edges, respectively, of $G$. The idea is to rely on the DFS-based framework introduced by Kosinas [ESA'23], for handling connectivity queries in the presence of multiple vertex failures. Our technical contribution is to show how to appropriately extend the toolkit of the DFS-based parameters, in order to optimally handle up to three vertex failures. Our approach has the interesting property that it does not rely on a compact representation of vertex cuts, and has the potential to provide optimal solutions for more vertex failures. Furthermore, we show that the DFS-based framework can be easily extended in order to answer vertex-cut queries, and the number of connected components in the presence of multiple vertex failures. In the case of three vertex failures, we can answer such queries in $O(\log n)$ time.

==> table3.tex <==
\hspace*{-0cm}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 {} & Preprocessing & Space & Update & Query\\ \hline\hline
 {Kanevsky et al.~\cite{}} & near linear & $O(n)$ & $-$ & $O(1)$\\ \hline
  
\end{tabular}

